A Survey of Spatio-Temporal EEG data Analysis: from Models to Applications

In recent years, the field of electroencephalography (EEG) analysis has witnessed remarkable advancements, driven by the integration of machine learning and artificial intelligence. This survey aims to encapsulate the latest developments, focusing on emerging methods and technologies that are poised to transform our comprehension and interpretation of brain activity. We delve into self-supervised learning methods that enable the robust representation of brain signals, which are fundamental for a variety of downstream applications. We also explore emerging discriminative methods, including graph neural networks (GNN), foundation models, and large language models (LLMs)-based approaches. Furthermore, we examine generative technologies that harness EEG data to produce images or text, offering novel perspectives on brain activity visualization and interpretation. The survey provides an extensive overview of these cutting-edge techniques, their current applications, and the profound implications they hold for future research and clinical practice. The relevant literature and open-source materials have been compiled and are consistently being refreshed at \url{https://github.com/wpf535236337/LLMs4TS}

==> 6_application_and_implications.tex <==
Applications and Implications
Clinical Applications: Discuss the impact of these advanced techniques on clinical practices, such as diagnosing neurological disorders.
Brain-Computer Interfaces (BCIs): Explore the role of advanced EEG analysis in enhancing BCI technologies.
Future Research Directions: Suggest potential areas for future research, based on the survey findings.
